GPU Scheduler for De Novo Genome Assembly with Multiple MPI Processes

$\textit{De Novo}$ Genome assembly is one of the most important tasks in computational biology. ELBA is the state-of-the-art distributed-memory parallel algorithm for overlap detection and layout simplification steps of $\textit{De Novo}$ genome assembly but exists a performance bottleneck in pairwise alignment. In this work, we proposed 3 GPU schedulers for ELBA to accommodate multiple MPI processes and multiple GPUs. The GPU schedulers enable multiple MPI processes to perform computation on GPUs in a round-robin fashion. Both strong and weak scaling experiments show that 3 schedulers are able to significantly improve the performance of baseline while there is a trade-off between parallelism and GPU scheduler overhead. For the best performance implementation, the one-to-one scheduler achieves $\sim$7-8$\times$ speed-up using 25 MPI processes compared with the baseline vanilla ELBA GPU scheduler.

==> fig/onetoonempi.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.33\columnwidth]{fig/onetoonempi.png}
\includegraphics[width=.33\columnwidth]{fig/onetoallmpi.png}
\end{center}
\caption{
\textbf{Outline -- }
A figure summarizing the entire algorithm
}
\label{fig:onetoonempi}
\end{figure*}

